DeepSpeed-Chat: Easy, Fast and Affordable RLHF Training of ChatGPT-like Models at All Scales

ChatGPT-like models have revolutionized various applications in artificial intelligence, from summarization and coding to translation, matching or even surpassing human performance. However, the current landscape lacks an accessible, efficient, and cost-effective end-to-end RLHF (Reinforcement Learning with Human Feedback) training pipeline for these powerful models, particularly when training at the scale of billions of parameters. This paper introduces DeepSpeed-Chat, a novel system that democratizes RLHF training, making it accessible to the AI community. DeepSpeed-Chat offers three key capabilities: an easy-to-use training and inference experience for ChatGPT-like models, a DeepSpeed-RLHF pipeline that replicates the training pipeline from InstructGPT, and a robust DeepSpeed-RLHF system that combines various optimizations for training and inference in a unified way. The system delivers unparalleled efficiency and scalability, enabling training of models with hundreds of billions of parameters in record time and at a fraction of the cost. With this development, DeepSpeed-Chat paves the way for broader access to advanced RLHF training, even for data scientists with limited resources, thereby fostering innovation and further development in the field of AI.

==> Makefile <==
PAPER=main

all: pdf
pdf: $(PAPER).pdf

SECTIONS = \
	evaluation.tex

TEXT = $(SECTIONS) 

TEX = main.tex \
        $(TEXT)

$(PAPER).bbl: references.bib
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

$(PAPER).pdf: $(TEX) $(FIGS) $(PAPER).bbl
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

clean:
	/bin/rm -f $(PAPER).aux $(PAPER).bbl $(PAPER).blg $(PAPER).dvi \
	$(PAPER).log $(PAPER).ps $(PAPER).pdf $(PAPER).out



